PatchMatch-RL: Deep MVS with Pixelwise Depth, Normal, and Visibility

Recent learning-based multi-view stereo (MVS) methods show excellent performance with dense cameras and small depth ranges. However, non-learning based approaches still outperform for scenes with large depth ranges and sparser wide-baseline views, in part due to their PatchMatch optimization over pixelwise estimates of depth, normals, and visibility. In this paper, we propose an end-to-end trainable PatchMatch-based MVS approach that combines advantages of trainable costs and regularizations with pixelwise estimates. To overcome the challenge of the non-differentiable PatchMatch optimization that involves iterative sampling and hard decisions, we use reinforcement learning to minimize expected photometric cost and maximize likelihood of ground truth depth and normals. We incorporate normal estimation by using dilated patch kernels, and propose a recurrent cost regularization that applies beyond frontal plane-sweep algorithms to our pixelwise depth/normal estimates. We evaluate our method on widely used MVS benchmarks, ETH3D and Tanks and Temples (TnT), and compare to other state of the art learning based MVS models. On ETH3D, our method outperforms other recent learning-based approaches and performs comparably on advanced TnT.

==> tex/old/detailed_method.tex <==
\section{Approach}
We propose \MethodName, an end-to-end learning framework that uses PatchMatch for Multi-View Stereo (MVS) reconstruction. 
In this section, We briefly review the PatchMatch MVS, introduce our approach, network architecture and training details as follows.

\subsection{Review of PatchMatch MVS}
We start by reviewing the generalized PatchMatch MVS algorithm. 
Given set of images $\mathcal{I}$ and its corresponding camera poses $\mathcal{C} = (\mathcal{K}, \mathcal{E})$ with intrinsic $\mathcal{K}$ and extrinsic $\mathcal{E}=[\mathcal{R}, t]$ matrices, the goal of PatchMatch MVS is to recover the depth of the reference image $I_{ref}\in \mathcal{I}$ from a set of selected source images $I_{src} \subset \mathcal{I}$ that overlap with $I_{ref}$.
Typically, PatchMatch MVS contains following structure:
\begin{enumerate}
    \vspace{-0.5em}
    \item[(1)] \textbf{Initialization} of labels per each pixel in $I_{ref}$.
    \vspace{-0.5em}
    \item[(2)] \textbf{Propagation} of labels in the $I_{ref}$ that facilitates co-planar or similar depth of nearby pixels.
    \vspace{-0.5em}
    \item[(3)] \textbf{Update} of labels based on the cost evaluation between $I_{ref}$ and the selected views of $I_{src}$. 
    %We show that a per-pixel joint view selection and cost regularization can be achieved via our reinforcement learning based approach. This helps avoid error matches due to local occlusion from a certain view. \TODO{better to have a small image illustration here?}.
\end{enumerate}
\textbf{Propagation} and \textbf{Update} steps are repeated fixed number of iterations, or until the labels are converged. We call the combined steps as PatchMatch iteration. 

\textbf{Initialization}. 
In the initialization stage, random oriented points are assigned for each pixels in the $I_{ref}$. 
An oriented point contains a depth and a normal value, which are independently initialized, and can be represented by the plane parameters  $\omega_p=[\textbf{n}^T_p; \delta_p]$, with the normal $\textbf{n}_p = [\textbf{n}_x, \textbf{n}_y, \textbf{n}_z]_p$ and disparity $\delta_p$ for each pixel $p \in I_{ref}$. 
Note that the oriented point $\omega_p$ can be related to depth $d_p$ as a line-plane intersection distance $d_p = -\delta_p / (n_p \cdot \mathcal{K}^{-1}\cdot p)$.

The depth $d_p$ of a pixel $p \in I_{ref}$ is initialized as: $d^0_p \sim 1/\mathcal{U}(\frac{1}{d_{max}}, \frac{1}{d_{min}})$, with $d_{min}$ and $d_{max}$ specifying the depth range. %e.g. set according to sparse points obtained during image registration. 
The depth range is reversed to prioritize the depths closer to the camera center over far away depths, as shown effective by Gallup \etal~\cite{galliani2015massively}. 
The per-pixel normal $n_p$ is initialized by sampling from a 3D Gaussian and normalization~\cite{muller1959note}. %, following Muller \etal
The normal vector is reversed if it faces the same direction as the pixel ray. 


\input{figures/kernel}

\textbf{Propagation}. 
The oriented point map $\omega^i$ at $i$-th PatchMatch iteration is propagated according to the propagation kernel. A common kernel is the Red-Black propagation kernel by Galliani \etal~\cite{galliani2015massively}, as illustrated in Figure \ref{fig:red-black-kernel}. We let $\psi^{i}_{:, p} = \{\omega^i_{q} \mid q \in K(p) \} \cup \{{\omega^i_p}^{pert} \}$ to denote the set of candidate oriented points obtained by propagation kernel $K$ at pixel $p$, and by randomly perturbing current candidate. The propagation can be applied using a series of convolutional filters of one-hot encodings, with one values in positions that correspond to each neighbor according to $K$.

\textbf{Update}. 
The labels are updated based on the likelihood of each labels per pixels. 
The likelihoods are obtained by estimating the visibility of each source images per pixel, and aggregating the matching score between the reference and the visible source images. 
We use $\mathcal{V}^{\theta}(\omega_p;\mathcal{I}, \mathcal{C})$ to denote pixel-wise visibility estimation function, and  $\mathcal{S}^{\theta}(\omega_p;\mathcal{I}, \mathcal{C}, \mathcal{V})$ to denote matching score function, parameterized by $\theta$.
%Instead, 
% We train the view-selection function $\mathcal{V}^{\theta}$ and matching cost function $\mathcal{S}^\theta$ parameterized by $\theta$. 
For ease of notation, we let $\mathcal{V}(\omega^i_p), \mathcal{S}(\omega^i_p)$ to denote $\mathcal{V}^\theta(\omega^i_p; \mathcal{I}, \mathcal{C}), \mathcal{S}^\theta(\omega^i_p; \mathcal{I}, \mathcal{C}, \mathcal{V})$ as the matching costs of the pixel $p$ in the oriented point map $\omega^i_p$, given images $\mathcal{I}$, cameras $\mathcal{C}$, and selected views $\mathcal{V}$. 
%Conventional PatchMatch MVS systems use handcrafted pixel-wise view-selection and matching cost functions, such as heuristic filtering on multi-hypothesis cost-matrix~\cite{xu2019multi} and aggregating bilaterally weighted normalized cross correlation values across selected views~\cite{schoenberger2016mvs}.  

% Training $\mathcal{V}(\omega^i_p)$ and $\mathcal{S}(\omega^i_p)$ is difficult because a good solution may not be available within candidates of a given iteration, but over several iterations, a good set of parameters will lead to a good solution.  For this, we turn to reinforcement learning, a well-known training technique for when multiple steps are required to reach a desirable state, as illustrated below.

% 2) Architecture/Approach, 
%    a. CNN for photometric matching, 
%    b. coarse-to-fine, 
%    c. view selection, 
%    d. cost regularization (basically current 4.1-4.3), 
%    e. refinement and fusion
\subsection{Architecture}
Figure~\ref{fig:architecture} shows an overview of our approach. 
We start by extracting a CNN features using Siamese network for the reference and the source images. 
Then, we employ coarse-to-fine variant of PatchMatch MVS, where at each level, we run series of PatchMatch iterations that consists of pixel-wise view selection, propagation, regularized cost computation and label update. 
The labels are then upsampled to a finer level, which starts new series of PatchMatch iterations. 
The final label map obtained at the finest layer of the PatchMatch are then fused into a point cloud.
\subsubsection{Multi-Scale Feature Extraction and Raw Correlation}
We use a variant of Feature Pyramid Network(FPN) to extract CNN features for reference and source images. 
To make it memory efficient, we vary the number of output channels for different scale, having shallower feature channels for the higher-resolution feature maps. We denote $\mathcal{F}^s_p$ to denote feature vector for pixel $p$ at image $s$. 
Following the differentiable warping~\cite{yao2018mvsnet}, the feature maps can be warped according to the pixel-wise plane homographies from reference image $r$ to source image $s$ as $H^{r\rightarrow s}_{\omega_p} = \mathcal{K}_s\cdot (\mathcal{R}_{r \rightarrow s} - \frac{t_{r\rightarrow s}\textbf{n}_p^{T}}{\delta_p}) \cdot \mathcal{K}_r^{-1}$. 
% where $\mathcal{R}, t$ defines the camera rotation and translation according to the reference camera. 
With support window $\mathcal{W}^{\gamma, \alpha}_p$ of size $\gamma$ and dilation $\alpha$ centered at $p$, we define the raw correlation value $\mathcal{G}^s_{\omega_p}$ of the oriented point $\omega_p$ as the attention-aggregated group-wise correlation for matching feature vectors in the source image:
\begin{align*}
   \mathcal{A}^q_p &= \sigma(\frac{\mathcal{F}^{r}_p \cdot h}{\sqrt{||\mathcal{F}^{r}_p||_2}})_q, q\in \mathcal{W}^{\gamma, \alpha}_p \\
   \mathcal{G}^s_{\omega_p} &= \sum_{q} \mathcal{A}^q_p \cdot (\mathcal{F}^{r}_q \circledast \mathcal{F}^s_{H^{r \rightarrow s}_{\omega_p} \cdot q})
\end{align*}
We let $\circledast$ to denote group-wise feature vector correlation~\cite{xu2020learning}, $\mathcal{A}^q_p$ as scaled dot-product attention for supporting pixel $q$ on center pixel $p$ by the reference feature map, and $h$ to represent attentional feature projection vector.
The resulting $\mathcal{G}^s_{\omega_p}$ represents the crude similarity between the feature patches between the reference and the source image at pixel $p$ and its oriented point candidate $\omega_p$. Figure~\ref{fig:group_correlation} illustrates how we obtain the raw correlation from the CNN features and the planar homographies. 

\input{figures/view_selection}
\subsubsection{Pixel-wise View Selection}
\label{sec:pixelwise_view_selection}
Following~\cite{schoenberger2016mvs}, we compute scale, incident-angle and triangulation angle difference based geometric priors for all source images for each pixel-wise plane $\omega_p$. 
Instead of hand-crafting the prior function, we concatenate the priors with the raw correlations $\mathcal{G}^{s}_{\omega_p}$ and use multi-layered perceptions(MLP) to learn a pixel-wise visibility estimate for each images $\hat{\mathcal{V}}^s_p \in [0, 1]$.
Figure~\ref{fig:view-selection} shows an example of the estimated visibilities in the source images.

We then sample $N$-views based on the L-1 normalized probability distribution over $\hat{\mathcal{V}}^s_p$ for each pixels, to obtain sampled set of views, $\mathcal{V}_p$. For estimating scores for each propagated candidates, we use both $\mathcal{V}_p$ and $\hat{\mathcal{V}}_p$ to compute the weighted raw correlation, $\mathcal{G}^{\mathcal{V}}_{\psi_{k, p}} = \frac{\sum_{v \in \mathcal{V}_p} \hat{\mathcal{V}}^{v}_p\mathcal{G}^v_{\psi_{k,p}} }{ \sum_{v\in \mathcal{V}_p} \hat{\mathcal{V}}^v_p}$, as a weighted mean of the aggregated group correlation for each patches. 

Because L-1 normalization minimizes scores of good source views that are not selected, as an robust training strategy, we use worst $M$-views along with selected $N$ views when we compute the L-1 probability of selecting the $N$ views for back-propagation. 

\subsubsection{Candidate Evaluation with Recurrent Cost Regularization}
%\subsubsection{Recurrent Cost Regularization}
Existing learning based cost regularization methods, such as 3D convolution on spatially aligned cost volume~\cite{yao2018mvsnet}, or $k$-nearest neighbor based graph convolutions~\cite{chen2019point}, exploits ordinals between each candidates for denoising the raw costs. However, our oriented point candidates are challenging to enforce such hierarchy between spatial neighbors. 
Instead, we get insight from loopy Belief-Propagation (LBP), where each node's belief is iteratively updated by message-passing from the neighboring nodes.  
The key insight is that node with high belief will less likely to be replaced by different candidates. 
We represent such belief to each oriented point candidates as hidden states $\zeta^i_{\psi_{k, p}}$, and use recurrent neural network(RNN) to estimate regularized score $\mathcal{Z}_{\psi_{k, p}}$ and updated hidden state $\zeta^{i+1}_{\psi_{k, p}}$. 

Similar to LBP, we compute pairwise neighborhood smoothness measure~\cite{besse2012pmbp} of the candidate oriented point in respect to the current label, $\{ M(\psi_{k, p}, \omega_q) | q \in \mathcal{N}(p) \}$, where $M(\omega_p, \omega_q) = Proj(\omega_p, q) + Proj(\omega_q, p)$ measures the similarity of the oriented points through the projection distances of the points on the plane formed from the oriented points.
We append the computed smoothness terms to the weighted raw correlation $\mathcal{G}^{\mathcal{V}}_{\psi_{k, p}}$, as an input to the RNN.
We update candidates for each pixel based on the resulting regularized scores for each candidates, and update the corresponding hidden states  as:
\begin{align*}
    \omega^{i+1}_p &= \psi_{k, p} \sim \mathcal{Z}_{\psi_{:, p}}\\
    \zeta^{i+1}_p &= \zeta^i_{\omega^{i+1}_{p}}
\end{align*}
The updated hidden states are used as an input to the recurrent cost regularization module in the next PatchMatch iteration. 

%\subsubsection{Coarse-to-Fine PatchMatch}
\textbf{Coarse-to-Fine PatchMatch.}
The estimated oriented point map $\omega^i$ and the hidden state map $\zeta^i$ are upsampled as an input to the finer level PatchMatch iteration. 
We use nearest neighbor interpolation where corresponding pixels in the upsampled region are assigned with the same label and hidden state values from the coarser stage. 

%\subsubsection{Fusion}
\textbf{Fusion.}
Given oriented point map estimates for each images, we follow the method used by other MVS literatures~\cite{yao2018mvsnet, galliani2015massively}, where first iterate each views as reference image to check the geometric consistency along with the source views. 
We check re-projection distance, and absolute point distance as a way to check whether the depth value is consistent across multiple views. 
Then, we re-project the mean value of $N$-view consistent depths into the world space to obtain the final point cloud. 


\section{Training with Reinforcement Learning}
There are challenges in making PatchMatch MVS end-to-end trainable: the $\arg\max$ based hard decisions/sampling required for PatchMatch update and view selection is non-differentiable; the incorporation of normal hypotheses is not trivial, since Soft-$\arg\max$ of oriented points makes the expectation of depth and normal to be dependent to each other. 
We propose a reinforcement learning approach to jointly learn matching cost and visibility estimation function.
Our formulation contains two agents, where one selects view and the other selects the candidates. 


\subsection{Reward Function}
We define the reward $r^t = \mathcal{N}(\omega^t; \omega^*, \sigma_\omega)$ as a probability of observing the oriented point from distribution given ground truth oriented point value $\omega^*$. We define the distribution as a joint independent normal distributions of depth and normal of pixel $p$:
\begin{equation}
    \mathcal{N}(\omega^t_p; \omega^*_p, \sigma_\omega) = \mathcal{N}(n^t_p; n^*_p, \sigma_n) \cdot \mathcal{N}(d^t_p; d^*_p, \sigma_d)
\end{equation}
We let expected future reward to be a $\gamma$-discounted sum of future rewards:  $G^t = \sum_{t' >= t} \gamma^{t'- t} r^t$. 
We can formulate the gradient of the reward to be a negation of the gradient of cross-entropy between the step-wise reward $\mathcal{N}(\omega^t; \omega^*, \sigma_\omega)$, and an agent $\pi_\theta(a^t, s^t)$, according to REINFORCE algorithm as:
\begin{align}
    \triangledown_\theta J &= \mathrm{E}_{\pi_\theta}[Q^{\pi_\theta}(s, a) \triangledown_\theta \log \pi_\theta(a \mid s)]\nonumber\\
    &= \sum_t \triangledown_\theta \ln \pi^t_\theta(a^t \mid s^t) G^t\nonumber\\
    &= \sum_t \sum_{t'>=t} \triangledown_\theta \gamma^{t'-t}(\mathcal{N}(\omega^{t'}; \omega^*, \sigma_\omega) \log \pi_\theta)
\end{align}

The sampling can be done through the categorical distribution, which makes the policy to approximate the expectation of the distribution, or argmax, which makes the policy to be the greedy solution. As an exploration versus exploitation strategy, we employ decaying $\epsilon$-greedy approach where we sampling candidates using expectation by probability of $\epsilon$ or using argmax by probability of $1 - \epsilon$. 

Below we describe the policy of each agent. We use $\mathbb{S}_\mathcal{V}, \mathbb{A}_\mathcal{V}, \pi_\mathcal{V}, \mathbb{R}_\mathcal{V}$, and $\mathbb{S}_\mathcal{S}, \mathbb{A}_\mathcal{S}, \pi_\mathcal{S}, \mathbb{R}_\mathcal{S}$ to denote the state, action, policy and reward space of the view selection and candidate selection agents respectively. For simplicity, we use $s^i \in \mathbb{S}$, $a^i \in \mathbb{A}$, and $r^i \in \mathbb{R}$ to denote the corresponding agent's state, action, and reward in the $i$-th iteration that apply to a particular pixel. 

\subsection{Learning Photometric Cost}
For the candidate selecting agent, the state space is the set of plane parameters for each oriented points $\omega_p$; the action space is the selection of a candidate label for each pixel in each iteration; and the policy encapsulates the parameterized cost function $\mathcal{S}(\omega^i_p)$.

Then, we can define the stochastic policy %$\pi_\mathcal{V}$ and 
$\pi_\mathcal{S}$ as a sampling function from distribution formed by action space:
\begin{align}
    \pi_\mathcal{S}(a^i \mid s^i) &= \omega^t \sim
    \frac{e^{-\mathcal{S}(\psi^i_:)}}{\sum_{q \in K} e^{-\mathcal{S}(\psi^i_q)}}
    \label{eq:policy_candidate}
\end{align}
which can be learned via gradient ascent:
\begin{align}
    \triangledown_\theta \log \pi_\mathcal{S}
    &= \triangledown_\theta 
        \log(
            \frac{e^{-\mathcal{S}(\omega^{i+1})}}
                 {\sum_{j \in K} e^{-\mathcal{S}(\psi^i_{j})}})\nonumber\\
    &= \triangledown_\theta (-\mathcal{S}(\omega^{i+1}) + \log \sum_{j \in K} e^{-\mathcal{S}(\psi^{i}_{j})})
    \label{eq:policy_gradient_candidate}
\end{align}

\subsection{Learning View Selection}
For the view selection agent, the state space represents set of source images; the action space is a selection of $N$ images among the source images for each iteration; and the policy uses the parameterized view selection function $\mathcal{V}(\omega^i_p)$. %Similarly,
The stochastic policy $\pi_\mathcal{V}$ is:
%Then, we can define the stochastic policy $\pi_\mathcal{V}$ and $\pi_\mathcal{S}$ as a sampling function from distribution formed by action space:
\begin{align}
    \label{eq:policy_view}
    \pi_\mathcal{V}(a^i \mid s^i) &= v \sim \frac{\hat{\mathcal{V}}^:}
         {\sum_{s \in \mathcal{I}} \hat{\mathcal{V}}^s}
\end{align}
and the gradient:
%and use Equations \ref{eq:policy_candidate} and \ref{eq:policy_view} to compute the gradient. 
%Because the reward is differentiable regarding the parameters $\theta$, we are able to directly train the PatchMatch MVS by gradient ascent to maximize reward. 
\begin{align}
    \triangledown_\theta \log \pi_\mathcal{V}
    &= \triangledown_\theta \log(
        \frac{\sum_{v\in \mathcal{V}}\hat{\mathcal{V}}^v}
             {\sum_{s \in \mathcal{I}} \hat{\mathcal{V}}^s})\nonumber \\
    \label{eq:policy_gradient_view}
    &\approx \triangledown_\theta 
        \log(\sum_{v\in \mathcal{V}}\hat{\mathcal{V}}^v) - 
        \log(\sum_{m \in M} \hat{\mathcal{V}}^m)
%    \triangledown_\theta \log \pi_\mathcal{S}
%    &= \triangledown_\theta 
%        \log(
%            \frac{e^{-\mathcal{S}(\omega^{i+1})}}
%                 {\sum_{j \in K} e^{-\mathcal{S}(\psi^i_{j})}})\nonumber\\
%    &= \triangledown_\theta (-\mathcal{S}(\omega^{i+1}) + \log \sum_{j \in K} %e^{-\mathcal{S}(\psi^{i}_{j})})
%    \label{eq:policy_gradient_candidate}
\end{align}
As mentioned in the section~\ref{sec:pixelwise_view_selection}, we use the selected N views, along with the M worst views for training the agent, to prevent the probabilities of the good, unselected views from being minimized. 
%Equations \ref{eq:policy_gradient_view} and \ref{eq:policy_gradient_candidate} are trivially differentiable, allowing end-to-end training.

==> tex/old/method.tex <==

\section{Implementation}
In this section, we propose an implementation of the MVS algorithm based on section \ref{sec:algorithm}.
Figure \ref{fig:architecture} provides an overview of our method.  We adopt the existing PatchMatch MVS architecture as a form of a coordinate descent~\cite{galliani2015massively,zheng2014patchmatch,schoenberger2016mvs,xu2019multi}, where we fix the plane-maps when estimating the view-selection and fix view-selection when updating the plane-maps. 
We start by extracting out multi-scale features using a shared CNN backbone. 
Then, we perform PatchMatch iterations by estimating pixel-wise weighted view selection given current plane-maps, 
propagating candidates, and updating scores from recurrent cost regularization. 
After a fixed number of iterations, we finally estimate per-pixel confidences, which are used in the off-line refinement process.

\subsection{Feature Extraction and Raw Correlation}
Inspired by Feature Pyramid Network~(FPN)~\cite{lin2017feature} which was shown to be effective in multi-scale consistent CNN features, we adopt a variant of FPN for the features used in coarse-to-fine PatchMatch MVS architecture, where number of feature channels at higher scale are reduced to be more memory efficient. 
For all images $\mathcal{I}$, we extract out feature maps $\mathcal{F}$ at different scales relative to the original image size. The features are extracted once, and shared throughout the PatchMatch iterations. 

Following the differentiable warping~\cite{yao2018mvsnet}, the feature maps can be warped according to the pixel-wise plane homographies $H_{\omega_p} = \mathcal{K}\cdot (\mathcal{R} - \frac{t - n_p^{T}}{\delta_p}) \cdot \mathcal{K}^{-1}$, where $\mathcal{R}, t$ defines the camera rotation and translation according to the reference camera. 
With support window $\mathcal{W}^{\gamma, \alpha}_p$ of size $\gamma$ and dilation $\alpha$ centered at $p$, we define the raw correlation value $\mathcal{G}_{\omega_p}$ of the plane $\omega_p$ as the attention-aggregated group-wise correlation for matching source feature vectors:
\begin{align*}
   \mathcal{A}^q_p &= \sigma(\frac{\mathcal{F}^{ref}_p \cdot h}{\sqrt{s}})_q, q\in \mathcal{W}^{\gamma, \alpha}_p \\
   \mathcal{G}_{\omega_p} &= \sum_{q} \mathcal{A}^q_p \cdot GroupCorr(\mathcal{F}^{ref}_q, \mathcal{F}_{H_{\omega_p} \cdot q})
\end{align*}
We let $\mathcal{F}^{ref}$ to denote reference feature map and $GroupCorr$ to denote group-wise correlation~\cite{Guo_2019_CVPR}.
$\mathcal{A}^q_p$ denotes scaled dot-product attention for supporting pixel $q$ on center pixel $p$ by the reference feature map, where $h$ represents attentional feature projection vector, and $s$ refers to feature vector dimension.
Figure~\ref{fig:group_correlation} illustrates how we obtain the raw correlation from the CNN features and the planar homographies. 

\subsection{Pixel-wise View Selection}
Pixel-wise visibility is a long-standing problem in the MVS literatures. We adopt a philosophy of existing state of the art architectures~\cite{zheng2014patchmatch, schoenberger2016mvs, xu2019multi} which computes pixel-wise view selection using current plane map, and update the plane map using the computed pixel-wise view selection for every iteration. Figure~\ref{fig:view-selection} describes our process of view selection. Following~\cite{schoenberger2016mvs}, we compute resolution, incident-angle and triangulation angle based geometric priors given our current plane map $\omega_p$. Instead of hand-crafting the prior function, we concatenate priors with the raw-patch correlations $\mathcal{G}_{\omega_p}$ and use multi-layered perceptions to learn a visibility estimate $\mathcal{V}_p$. We then sample $N$-views based on $\mathcal{V}_p$ for each pixels. We keep the visiblity estimate $\mathcal{V}_p$ to compute the weighted raw correlation, $\mathcal{G}^{\mathcal{V}}_{\omega_p}$, which computes weighted mean of the aggregated group correlation for each patches. To train pixel-wise visibility, we use reward-driven training described in section \ref{sec:algorithm}.

\subsection{Candidate Evaluation with Recurrent Cost Regularization}
Cost filtering using cost-volume regularization has been widely adopted in the learning based MVS literatures~\cite{yao2018mvsnet,yao2019recurrent,chen2019point,luo2020attention}, which is known to reduce raw cost noises using 3D convolution filters. 
However, the existing works on cost-volume regularization assumes that the costs are spatially aligned, which is not possible in the PatchMatch based or plane-map based architectures. 
Instead, we find the iterative nature of the PatchMatch to be closely related to the recurrent neural network (RNN) architecture, and thus propose a form of regularization as a regularize-through-time. Figure~\ref{fig:regularization} describes our recurrent cost regularization process. 
For every plane $\omega^t_p$, we assign hidden state $\mathcal{H}^t_p$, that are zero-initialized at time $t=0$. 

Then, we define RNN based cost regularization where it takes raw patch correlations for all propagated planes $\mathcal{G}^{\mathcal{V}}_{\omega^t_q}, q\in K(p)$ and hidden states $\mathcal{H}^t_p$ to output regularized cost $\mathcal{Q}_{\omega^t_q}$ and estimated hidden states $\mathcal{H}^{t}_{q, p}$ for candidate $q$.
Following the PatchMatch update, we sample the best plane $\omega^{t+1}_p = \mathrm{argmax}_{q} \mathcal{Q}_{\omega^t_q}$ and its corresponding hidden state $\mathcal{H}^{t+1}_p = \mathcal{H}^{t}_{\mathrm{argmax}_q, p}$.
Recurrent cost regularization can also be viewed as a form of loopy belief propagation, where the hidden states represents a current belief on the node $p$.

\subsection{Coarse-to-Fine Up-Scaling}
Following \cite{xu2019multi}, which has shown the efficiency and robustness of the coarse-to-fine architecture, after fixed number of iterations per each scale, the plane map and the hidden states are up-scaled with nearest neighbor interpolation. Note that the policy gradient can be trained through multiple scales by up-scaling the reward with the same interpolation scheme. 

\subsection{Refinement and Fusion}
Given final plane-map, we estimate the confidence of the plane map by shallow layers of CNN, using the concatenation of $n_p$, $Q_p$ and $\mathcal{I}_p$ as input. We follow \cite{rossi2020joint, kuhn2019deepc} where we jointly refine the depth and normal map as a confidence-mask based optimization. This refinement process is known to fill in the unconfident regions through plane propagation. 
Finally, we follow the fusion process of \cite{galliani2015massively, yao2018mvsnet}, where depth of each views are back-projected, and eliminated if the depth is inconsistent with at least 2 number of views. The inconsistency is measured by re-projection distances, normal consistency and absolute depth difference. 

% The matching costs of each plane candidates at the PatchMatch propagation are evaluated by the function $F^\theta$, which are defined by trainable parameters $\theta$. 
% We follow the VA-Point-MVSNet, \cite{chen2019point}, mainly, the $vis-var$ based aggregation that uses visibility-weighted variance of features for variance-based metric that Yao et al. \cite{yao2018mvsnet} proposed. 
% Because the visibility mask is not available during PatchMatch iteration, as VA-Point-MVSNet computes it through coarse plane-sweep to estimate initial visibility map, we use the geometric prior values, and feature similarity to estimate the view-selection weights.

% Figure \ref{fig:view-selection-weighting} and  \ref{fig:weighted-variance} describe our view-weighted variance based scoring function. 
% We start by extracting CNN features, which are pixel-wise warped based on the depth values of the current iteration. 
% To further improve the impact of the geometric priors, we follow \cite{mildenhall2020nerf} to map the geomtric prior values into higher dimensional features, by using positional encoding.
% The warped features are concatenated together along with the encoded geometric prior values, which are passed on to MLP followed by Sigmoid to output visibility value in $[0, 1]$. 
% Finally, We use the view-selection weights to obtain channel-wise weighted variance, which the multi-patch similarity MLP layers evaluate into final scores for each depth. 


==> tex/old/notation.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{rcp{6cm} }
    \toprule 
    $\textbf{n}^i_p$ & $\triangleq$& 
    Plane Normal (at pixel $p$, at $i$-th iteration of PatchMatch)\\
    
    $d^i_p$     & $\triangleq$& 
    Depth \\
    
    $\delta^i_p$     & $\triangleq$& 
    Origin-Plane distance\\
    
    $\omega^i_p$     & $\triangleq$&
    Plane $=$ $[\textbf{n}_p^{T} \delta_p]$\\
    
    $K$     & $\triangleq$&
    PatchMatch Propagation Kernel\\
    
    $\psi^i_{k, p}$     & $\triangleq$&
    $k$-th propagated plane\\
    
    
    $\mathcal{W}^{\gamma,\alpha}_p$     & $\triangleq$&
    Support Window for the plane at $p$, with size $\gamma$ and dilation $\alpha$\\
    
    
    $\mathcal{I}_s$     & $\triangleq$&
    Image $s$ from set of image $\mathcal{I}$\\
    
    $\mathcal{K}$     & $\triangleq$&
    Camera intrinsics\\
    
    $\mathcal{E}$     & $\triangleq$&
    Camera extrinsics $=$ ($\mathcal{R}, t)$\\
    
    $\mathcal{C}$     & $\triangleq$&
    Cameras $=$ ($\mathcal{K}, \mathcal{E}$)\\
    
    $\mathcal{H}^{r \rightarrow s}_{\omega_p}$     & $\triangleq$&
    Plane homography using $\omega_p$ $=$ $\mathcal{K}_s (\mathcal{R}_s\mathcal{R}^{T}_{r}- \frac{(-\mathcal{R}_s \mathcal{R}^{-1}_r t_r + t_s)\textbf{n}^T}{\delta_p})\mathcal{K}_r$\\
    
    $\mathcal{F}^s_p$ & $\triangleq$ &
    Feature vector at image $s$ at pixel $p$\\
    
    $\mathcal{A}^q_p$ & $\triangleq$ &
    Bilateral, dot-scaled attention for support windows pixels $=$ 
    $\sigma(\frac{\mathcal{F}^r_p \cdot h}{\sqrt{||\mathcal{F}^r_p||_2}})$ , $h$ $=$ attention projection vector\\
    
    $\mathcal{G}^s_{\omega_p}$ & $\triangleq$ &
    Attention-aggregated Group Correlation between $\mathcal{F}^r_q$ and $\mathcal{F}^s_{\mathcal{H}^{r \rightarrow s}_{\omega_p}q}$ for $q\in \mathcal{W}_p$\\
    
    
    \bottomrule
    \end{tabular}
    \caption{Notation Table for Detailed Architecture}
    \label{tab:notation}
\end{table}


==> tex/old/patchmatch_iterations.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{images/architectures/patchmatch_iterations.png}
    \caption{
        \textbf{An Example of single PatchMatch iteration.}
        Our PatchMatch iteration consists of three stages: Pixel-wise view selection, candidate propagation, and candidate selection. 
        Pixel-wise view selection uses the geometric priors with raw feature correlation to choose which view to score the candidates. 
        Candidate propagation generates multiple candidates per pixel using PatchMatch propagation along with small local plane perturbations. 
        Finally, candidate selection chooses candidates based on the regularized scores obtained from the selected views.
    }
    \label{fig:patchmatch_iterations}
 \end{figure*}


==> tex/old/score_selection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{images/vanilla_patch_match.png} \\
    \includegraphics[width=0.47\textwidth]{images/duggal_et_al.png} \\
    \includegraphics[width=0.47\textwidth]{images/our_update.png}\\
    \caption{\textbf{Comparison of Score Updates}. The top row indicates the method used by vanilla PatchMatch MVS algorithms. The method takes the argmax along the propagation. The mid-row indicates the work by Duggal et al\cite{duggal2019deeppruner}, which uses soft-argmax based aggregation. The last row indicates our method, which chooses depth by using sampling through softmax distribution.
    }
    \label{fig:score_update}
 \end{figure}


==> tex/old/view_selection_weights.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{images/view-selection_weights.png}
    \caption{
    \textbf{View-Selction Weight computation.}
    We use the feature vector at reference pixel, and warped source pixels according to the depth, concatenated with positional encoded features to obtain view-selection weights.
    We use MLP to estimate weights on how much the source pixel should be used for contributing to compute the scores for the depth value.}
    \label{fig:view-selection-weighting}
 \end{figure}


==> tex/old/weighted_variance.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{images/weighted_variance.png}
    \caption{
    \textbf{Weighted Variance based scoring.}
    We use weighted variance in order to obtain the final score. The weights were obtained through the view-selection weights. We use the same feature concatenation to compute the weighted channel-wise variance of the features. Then, the weighted variance is passed into MLP to estimate the final score $s$.
    }
    \label{fig:weighted-variance}
 \end{figure}


==> tex/prelimiaries.tex <==
\section{Algorithm}
\label{sec:algorithm}
In this section, we derive PatchMatch MVS into a reinforcement learning problem. 
We start by reviewing the PatchMatch MVS algorithm, followed by overview of the policy gradient algorithm. Then, we formulate PatchMatch algorithm as a reinforcement learning problem. 

\subsection{Review of the PatchMatch Multi-View Stereo}
PatchMatch~\cite{generalized_patchmatch} optimizes a randomly initialized label or correspondence map by iteratively propagating, evaluating, and selecting candidates from perturbations and neighboring pixel hypotheses. 
%PatchMatch  is  an  optimization  process  where  it  itera-tively updates the randomly initialized correspondence mapby  comparing  against  the  candidates  obtained  from  theneighbors. 
In application to multiview stereo (MVS), the label map consists of depth and/or normal values, and the propagation scheme favors that nearby pixels are co-planar or have similar depth. 
%PatchMatch MVS, is a variant of the generalized PatchMatch algorithm, where the correspondence is obtained through a scene space geometry, such as points or planes. 
We review the variant of PatchMatch MVS by Gallup \etal~\cite{galliani2015massively} that iteratively solves for plane $\omega_p$ for every pixel $p$ in the reference image $I_{ref}$.

PatchMatch MVS contains 3 steps: (1) Initialize, (2) Propagate, and (3) Update.
The planes are randomly initialized at the \textbf{Initialize} step. Then, the plane map $\omega$ is propagated according to the PatchMatch propagation kernel in the \textbf{Propagate} step, which are evaluated and updated based on scores in the \textbf{Update} step. A PatchMatch \textbf{iteration} consists of performing the Propogate and Update steps.

We define plane map $\omega^i=[n^i_p; \delta^i_p]$ to denote plane map at $i$-th PatchMatch iteration, parameterized by plane normal $n^i_p = [n_x, n_y, n_z]^i_p$ and disparity $\delta^i_p$, for each pixel $p$ for the reference image $I_{ref} \in \mathcal{I}$. 
We let $\mathcal{C} = (\mathcal{K}, \mathcal{E})$ to denote cameras with intrinsic $\mathcal{K}$ and extrinsic $\mathcal{E}$ matrices, and $F(\omega_p;\mathcal{I}, \mathcal{C})$ to denote matching function, for plane $\omega_p$ at pixel $p$ given images with known poses. Finally, we let $K(p)$ to denote PatchMatch kernel that defines a local neighborhood search space. The plane $\omega_p$ can be related to depth $d_p$ as a line-plane intersection distance $d_p = -\delta_p / (n_p \cdot \mathcal{K}^{-1}\cdot p)$. %, and vice versa $\delta_p = -d_p (n_p \cdot \mathcal{K}^{-1} \cdot p)$.

\textbf{Initialize: } Following Muller \etal~\cite{muller1959note}, each plane normal $n_p$ is initialized by sampling from a 3D Gaussian and normalizing. If the normal vector and pixel ray face the same direction, the normal vector is reversed. The depth $d_p$ is initialized as:
\begin{equation}
    d^0_p \sim 1/\mathcal{U}(\frac{1}{d_{max}}, \frac{1}{d_{min}})
\end{equation}
with $d_{min}$ and $d_{max}$ specifying the depth range, e.g. set according to sparse points obtained during image registration. We use inverse of depth ranges to prioritize depths that are closer to the camera center over far away regions, as shown effective by Gallup \etal~\cite{galliani2015massively}. 
\input{figures/kernel}

\textbf{Propagate: } New candidates for $\omega_p$ are propagated from pixels in the neighborhood defined by kernel $K$, as described in Figure~\ref{fig:red-black-kernel}. Evaluating more candidates can improve accuracy, but costs more computation and memory. We denote plane map $\omega^i$ propagated planes using kernel $K$ as $\Psi^i_K$, where $\psi^i_{k,p}$ indicates the plane at $p$ using the $k$th neighboring pixel:
\begin{equation}
    \psi^{i}_{:, p} = \{\omega^i_{q} \mid q \in K(p) \}
\end{equation} 
We implement the propagation as a series of convolutional filters of one-hot encodings, with one values in positions that correspond to each neighbor according to $K$.

\textbf{Update: } Each pixel is assigned the best propagated plane value by evaluating the matching cost function $F$.
\begin{equation}
    \omega^{i+1}_{p} = \underset{\psi^i_{k, p}}{\mathrm{argmax}}  F_p(\psi^i_{:, p}; \mathcal{I}, \mathcal{C}) \\
\end{equation} 
The matching cost function $F$ scores the likelihood that a pixel in the reference image corresponds to the candidate plane, given the source images. 
Conventional PatchMatch MVS systems use handcrafted matching cost function, such as aggregating bilaterally weighted normalized cross correlation values across selected views~\cite{schoenberger2016mvs}. 
Instead, we train the matching cost function $F^\phi$ parameterized by $\phi$. For ease of notation, we let $F(\omega^i_p)$ to denote $F^\phi(\omega^i_p; \mathcal{I}, \mathcal{C})$ as the matching costs of the pixel $p$ in the propagated plane map $\omega^i_p$, given images $\mathcal{I}$ and cameras $\mathcal{C}$. A fixed number of iterations of Propagate and Update are performed. 

Training $F(\omega^i_p)$ is difficult because a good solution may not be available within candidates of a given iteration, but over several iterations, a good set of parameters will lead to a good solution.  For this, we turn to reinforcement learning, a well-known training technique for when multiple steps are required to reach a desirable state. 

\subsection{Review of Policy Gradient}
Policy Gradient is a way to optimize over the reinforcement learning problem, searching for the optimal policy given the states. 
A typical reinforcement learning problem is described with states $S$, actions $A$, reward $R$ and policy $\pi$. 
The states and state-action pairs are evaluated as a function dependent on the policy $\pi$ as $V^\pi(s)$ and $Q^\pi(s, a)$ where $s\in S$ and $a \in A$. $V^\pi(s)$ represents the value of being in the state $s$ according to the policy $\pi$, and $Q^\pi(s, a)$ represents the value of choosing action $a$ in the state $s$ at given policy $\pi$. We parameterize $\pi$ with $\theta$, denoted as $\pi_\theta$.
Then, we can define the reward function $J(\theta)$ as an expected value function over all states:
\begin{align}
    J(\theta) &= \sum_{s\in S} d^{\pi_\theta}(s) V^{\pi_\theta}(s) \\
              &= \sum_{s\in S} d^{\pi_\theta}(s) \sum_{a\in A} \pi_\theta(a \mid s) Q^{\pi_\theta}(s, a) \\
\end{align}
where $d^{\pi_\theta}(s) = \lim_{t \rightarrow \infty} P(s_t=s \mid s_0, \pi_\theta)$ indicates the stationary Markov Chain distribution of $\pi_\theta$ on the state $s$.

The gradient of reward with respect to the parameters $\triangledown_\theta J(\theta)$ is computed as
\begin{align}
    \triangledown_\theta J(\theta) &= \triangledown_\theta \sum_{s\in S} d^{\pi_\theta}(s) \sum_{a\in A} \pi_\theta(a \mid s) Q^{\pi_\theta}(s, a) \\
                            &\propto \sum_{s\in S} d^{\pi_\theta}(s) \sum_{a\in A} Q^{\pi_\theta}(s, a) \triangledown_\theta \pi_\theta(a \mid s)  \\
                            &= \mathrm{E}_{\pi_\theta}[Q^{\pi_\theta}(s, a) \triangledown_\theta \ln \pi_\theta(a \mid s)]
\end{align}
Thus, we can train the parameters $\theta$ that will maximize the reward $J$ by running gradient ascent on $\triangledown_\theta J$, known as the policy gradient method.

\subsection{Training PatchMatch Multi-View Stereo using Policy Gradient}
To enable training the propagate/update steps, we formulate PatchMatch MVS as a reinforcement learning problem.  The state space $\mathcal{S}$ is the set of plane parameters for each pixel $\omega$; the action space $\mathcal{A}$ is the selection of a candidate plane for each pixel in each iteration; and the policy $\pi$ parameters $\theta$ are the parameters of the cost function $F(\omega^i_p)$ used to select a plane candidate. For simplicity, we use $s^t \in S$, $a^t \in \mathcal{A}$, and $r^t \in \mathcal{R}$ to denote the state, action, and reward in the $t$th iteration that apply to a particular pixel. 

%We use $s^i_p \in S^i_p$, $a^i_p \in \mathcal{A}^i_p$, and $r^i_p \in \mathcal{R}^i_p$ to describe the states, actions and rewards at time step $i$ for pixel $p$, and $\pi^\theta$ to denote the stochastic policy parameterized by $\theta$.
%For simplicity, we drop $p$ in the notation for the equations forward.
%We define the state space $\mathcal{S} \in (\mathcal{C} \times \mathcal{I} \times \Omega)$ to represent images, cameras and plane at current iteration, and action space $\mathcal{A} \in \Omega$ to be the updated value of the PatchMatch iteration. 

Then, we can define the stochastic policy $\pi_\theta$ as a sampling from distribution of matching costs of each plane values:
\begin{align}
    \pi_\theta(a^t \mid s^t) &= \mathrm{E}[\omega^t | \psi^t_{:}] \\
                         &= \omega^t \sim \frac{e^{F(\psi^t_{:})}}{\sum_{q \in K} e^{F(\psi^t_{q})}}
\end{align}
The plane $\omega^t$ is sampled from the categorical distribution of candidates from PatchMatch propagation $\psi^t$ at iteration $t$ for each pixel.
Unlike the original PatchMatch that selects the best score, or the differentiable PatchMatch that takes the soft-argmax value, our method takes the expectation of the score through sampling.

We define the reward $r^t = \mathcal{N}(\omega^t; \omega^*, \sigma_\omega)$ as a probability of observing plane from distribution given ground truth plane value $\omega^*$. We define the distribution as a joint independent normal distributions of depth and normal of pixel $p$:
\begin{equation}
    \mathcal{N}(\omega^t_p; \omega^*_p, \sigma_\omega) = \mathcal{N}(n^t_p; n^*_p, \sigma_n) \cdot \mathcal{N}(d^t_p; d^*_p, \sigma_d)
\end{equation}
Setting the discount factor $\gamma$ to 0 makes the expected future reward equal to the current reward: 
$G^t = r^t + \sum_{t' > t} \gamma^{t'} r^t = r^t$.  We can formulate the gradient of the reward to be a negation of the gradient of cross-entropy between $\mathcal{N}(\omega^t; \omega^*, \sigma_\omega)$, and $\omega_\theta(a^t, s^t)$, according to REINFORCE algorithm as:
\begin{align}
    \triangledown_\theta J(\theta) &= \mathrm{E}_{\pi_\theta}[Q^{\pi_\theta}(s, a) \triangledown_\theta \ln \pi_\theta(a \mid s)]\\
    &= \sum_t \triangledown_\theta \log \pi\theta(a^t \mid s^t) G^t\\
    &= \sum_t \triangledown_\theta (\mathcal{N}(\omega^t; \omega^*, \sigma_\omega) \log \pi_\theta(a^t \mid s^t))
\end{align}
and use Equation \ref{eq:policy} to compute the gradient. Because the reward is differentiable regarding the parameters $\theta$, we are able to directly train the PatchMatch MVS by gradient ascent to maximize reward. 
\begin{align}
    \triangledown_\theta \log \pi_\theta
    &= \triangledown_\theta \log(\frac{e^{F(\psi^t_{k, p})}}{\sum_{j \in K(p)} e^{F(\psi^t_{j,p})}}), \forall p \in \mathcal{I}\\
&= \triangledown_\theta (-F(\omega^t_p) + \log \sum_{j \in K(p)} e^{F(\psi^t_{j,p})})
\end{align}
Equation \ref{eq:policy_gradient} is trivially differentiable, allowing end-to-end training.
